A Divide-and-Conquer Algorithm for Betweenness Centrality

The problem of efficiently computing the betweenness centrality of nodes has been researched extensively. To date, the best known exact and centralized algorithm for this task is an algorithm proposed in 2001 by Brandes. The contribution of our paper is Brandes++, an algorithm for exact efficient computation of betweenness centrality. The crux of our algorithm is that we create a sketch of the graph, that we call the skeleton, by replacing subgraphs with simpler graph structures. Depending on the underlying graph structure, using this skeleton and by keeping appropriate summaries Brandes++ we can achieve significantly low running times in our computations. Extensive experimental evaluation on real life datasets demonstrate the efficacy of our algorithm for different types of graphs. We release our code for benefit of the research community.

==> conclusions.tex <==
In this paper, we proposed {\ouralgo} 
that computes for any given target
set $S$  the exact betweenness centrality of nodes. 
{\ouralgo} is a divide-and-conquer algorithm that splits the input graph into smaller 
subgraphs, applies the {\brandes} algorithms on these subgraphs and appropriately stores
and combines the results of these computations.
In our analysis and experimental evaluation on real data, we demonstrated that in many cases {\ouralgo}
achieves significant speedups over {\brandes}.
%For verifiability of our experiments as well as further scientific use we make our implementations available at:~\url{http://cs-people.bu.edu/edori/code.html}.

